rEGGression: an Interactive and Agnostic Tool for the Exploration of Symbolic Regression Models

Regression analysis is used for prediction and to understand the effect of independent variables on dependent variables. Symbolic regression (SR) automates the search for non-linear regression models, delivering a set of hypotheses that balances accuracy with the possibility to understand the phenomena. Many SR implementations return a Pareto front allowing the choice of the best trade-off. However, this hides alternatives that are close to non-domination, limiting these choices. Equality graphs (e-graphs) allow to represent large sets of expressions compactly by efficiently handling duplicated parts occurring in multiple expressions. E-graphs allow to store and query all SR solution candidates visited in one or multiple GP runs efficiently and open the possibility to analyse much larger sets of SR solution candidates. We introduce rEGGression, a tool using e-graphs to enable the exploration of a large set of symbolic expressions which provides querying, filtering, and pattern matching features creating an interactive experience to gain insights about SR models. The main highlight is its focus in the exploration of the building blocks found during the search that can help the experts to find insights about the studied phenomena.This is possible by exploiting the pattern matching capability of the e-graph data structure.

==> crossover.tex <==
\begin{tikzpicture}[scale=0.65,sibling distance=5em,
  every node/.style = {shape=circle,  draw, align=center, top color=white, bottom color=lightgray!20, minimum size=6mm,inner sep=0pt},
  level 1/.style={sibling distance=5em},
  level 2/.style={sibling distance=3em},
    ]]

  \node(first) {$+$}
          child { node  {$\mathbf{x}$} }
          child { node [thick, bottom color=lightgray!80] {$cos$}  
                    child { node {$x$}  }
                }

         ;

  \node(plus)[right= 0.7cm of first, draw=none, fill=none, bottom color=white] {}
       child  { [white] node[draw=none, fill=none, bottom color=white, black] {$+$} };
  
  \node(second)[right= 0.7cm of plus, thick, bottom color=lightgray!80] {$*$}
          child { node  {$+$} 
                    child {  node {$x$} }
                    child {  node [thick, bottom color=lightgray!80]{$2$} }
                }
          child { node {$x$} }

         ;
  \node(equal) [right= 0.7cm of second, draw=none, fill=none, bottom color=white]{}
       child  { [white] node[draw=none, fill=none, bottom color=white, black] {$=$} };

  \node(third)[right= 0.7cm of equal] {$+$}
          child { node  {$\mathbf{x}$} }
          child { node [thick, bottom color=lightgray!80] {$2$}  
                }

         ;
         
\end{tikzpicture}


==> mutation.tex <==
\begin{tikzpicture}[scale=0.65,sibling distance=5em,
  every node/.style = {shape=circle,  draw, align=center, top color=white, bottom color=lightgray!20, minimum size=6mm,inner sep=0pt},
  level 1/.style={sibling distance=5em},
  level 2/.style={sibling distance=3em},
    ]]

  \node(first) {$+$}
          child { node {$x$} }
          child { node [thick, bottom color=lightgray!80] {$\mathbf{cos}$}  
                    child { node {$x$}  }
                }

         ;
 
  \node(equal) [right= 0.7cm of first, draw=none, fill=none, bottom color=white]{}
       child  { [white] node[draw=none, fill=none, bottom color=white, black] {$=>$} }
  ;

  \node(third) [right= 0.7cm of equal] {$+$}
          child { node {$x$} }
          child { node [thick, , bottom color=lightgray!80] {$+$}  
                    child { node [thick, , bottom color=lightgray!80] {$2$} }
                    child { node [thick, , bottom color=lightgray!80] {$x$}  }
                }

         ;
    \node(equal2) [right= 0.7cm of third, draw=none, fill=none, bottom color=white]{}
       child  { [white] node[draw=none, fill=none, bottom color=white, black] {$=>$} }
  ;
    \node(fourth) [right= 0.7cm of equal2] {$+$}
          child { node {$x$} }
          child { node [thick, bottom color=lightgray!80] {$*$}   
                    child { node {$2$} }
                    child { node {$x$}  }
                }

         ;
\end{tikzpicture}
